Xing USP: A Cross-Family Semantic Contract for Information Extraction and Intent-Slot Parsing

Structured semantic parsing is typically judged by whether the correct category is assigned, which leaves value recovery and instance-level associations unexamined: a system may recognize an event yet bind an argument to the wrong instance, or identify an intent yet supply an incorrect slot value. We present USP, a cross-family semantic contract that represents categories, fields, values, and instance associations through a common interface for named-entity recognition, relation extraction, event extraction, and intent-slot parsing. The contract is paired with five diagnostic matching views---category agreement, field recognition, field-value pairing, instance-bound assignment, and complete-instance recovery---that ask distinct questions about the same output. Using this contract, we normalize 61 datasets into a unified corpus with shared schemas, prompts, and matching rules, and compare six models on a fixed test subset. Our fine-tuned Xing4.0-29B-Intent attains 57.70 task-balanced Field-Value Micro-F1 (equally weighted across the four task families) and ranks first in every family and on all five views; its margin over the strongest alternative widens from 2.93 points for category matching to 20.73 points for complete-instance matching. This widening gap shows that category agreement alone understates structural deficits. USP thus offers the community a shared representation, a normalized 61-dataset corpus, and a diagnostic evaluation protocol that make structural agreement measurable and comparable across extraction and intent-slot tasks.

==> tabs/biz_ablation.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{ll|ccc}
    \toprule
        Recipe & Backbone & Device A & Assistant & Device B$_{\text{hard}}$ \\
    \hline
        Base & TeleChat2.5-3B & 0.217 & 0.237 & 0.146 \\
        Base & TeleChat2.5-7B & 0.318 & 0.246 & 0.193 \\
        Base & Qwen3-4B       & 0.565 & 0.596 & 0.267 \\
        Base & Qwen3-8B       & 0.640 & 0.659 & 0.301 \\
        \hline
        SFT & 3B                  & 0.794 & 0.837 & 0.313 \\
        SFT & 7B                  & 0.840 & 0.858 & 0.417 \\
        SFT\,+\,warm-start & 7B    & 0.829 & 0.861 & 0.307 \\
        SFT\,+\,ratio-tuned & 7B   & 0.939 & 0.846 & 0.560 \\
        \textbf{SFT (best)} & \textbf{7B} & \textbf{0.954} & \textbf{0.883} & \textbf{0.640} \\
        SFT\,+\,8:1 ratio & 7B     & 0.868 & 0.849 & 0.550 \\
        SFT\,+\,RL warm-start & 7B & 0.851 & 0.867 & 0.577 \\
        SFT & Qwen3-8B            & 0.861 & 0.833 & 0.514 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{Recipe ablation for in-domain business SLU (strict intent+slot Equality-Accuracy). Scenarios are renamed (\emph{Smart Devices}/\emph{Smart Assistant}); recipe labels describe the knob only. The hard scenario (Device B) is the bottleneck throughout: $3$B$\to$7B helps most there ($0.313\to0.417$) and data ratio is the dominant lever ($0.417\to0.560\to0.640$), with $5{:}1$ domain:general beating $8{:}1$. Warm-start and RL warm-start raise the main scenarios but do not beat the best plain SFT. The same recipe on a Qwen3-8B backbone trails the best Xing-7B on the hard scenario ($0.514$ vs.\ $0.640$), a backbone$\times$recipe interaction consistent with the backbone-dependent alignment tax.}
    \label{tab:biz_ablation}
\end{table}


==> tabs/cold_start.tex <==
% =====================================================================
% SUSPENDED-TABLE-B4-COLDSTART (retired 2026-07-28).
% Numbers 0.454 / 0.348 / 0.597 trace to the retired exp5-era released
% checkpoint on an unreleased business intent set. Parent
% (acl_latex_v4.tex) currently wraps the \input{tabs/cold_start} call in
% \iffalse; if you re-\input this file from elsewhere, wrap the call in
% \iffalse ... \fi until the mechanical-identity fix lands.
% =====================================================================
\iffalse
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{6pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|cc}
    \toprule
        Model & Classification ACC & Extraction ACC \\
        \hline
        qwen2.5-7B (0-shot)            & 0.206 & 0.003 \\
        qwen3-8B (0-shot)              & 0.348 & 0.020 \\
        TeleChat2.5-7B (0-shot)        & 0.112 & 0.006 \\
        {\ours} (ours)                 & \textbf{0.454} & 0.017 \\
        \ \ + business/think data      & \textbf{0.597} & \textbf{0.029} \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Zero-shot diagnostic on an industry intent set with \emph{dynamic, unseen} schema (accuracy). \emph{Every} model---general and dedicated---collapses on slot \textbf{extraction} (ACC $\le$3\%), even when classification is moderate. This is the strongest evidence that current models do not solve schema-driven parsing under distribution shift, motivating {\ours}.}
    \label{tab:cold-start}
\end{table}
\fi
% END SUSPENDED-TABLE-B4-COLDSTART


==> tabs/indomain_biz.tex <==
% =====================================================================
% SUSPENDED-TABLE-B4-INDOMAIN (retired 2026-07-28).
%
% LINEAGE WARNING: this table reports an internal-data recipe on a
% telechat2.5-7B backbone with business-data SFT. It is DISTINCT from
% the open-data current intermediate candidate \ours checkpoint. The
% Equality-Accuracy figures 0.19-0.32 (base) and 0.64-0.95 (+business
% SFT) trace to unreleased business data and to a retired exp5-era
% candidate; they are held for the frozen-checkpoint re-run and must not
% be re-inhabited as open-data released-model results.
%
% Parent (acl_latex_v4.tex) currently wraps the \input{tabs/indomain_biz}
% call in \iffalse; if you re-\input this file from elsewhere, wrap the
% call in \iffalse ... \fi until the mechanical-identity fix lands.
% =====================================================================
\iffalse
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{5pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|cc|cc}
    \toprule
        \multirow{2}*{Scenario (renamed)} & \multicolumn{2}{c|}{Base TeleChat2.5-7B} & \multicolumn{2}{c}{+ business SFT} \\
        \cline{2-5}
         ~ & Intent & Int+Slot & Intent & Int+Slot \\
        \hline
        Smart Assistant        & 0.505 & 0.246 & \textbf{0.980} & \textbf{0.883} \\
        Smart Device A         & 0.455 & 0.318 & \textbf{0.969} & \textbf{0.954} \\
        Smart Device B (hard)  & 0.426 & 0.193 & \textbf{0.760} & \textbf{0.640} \\
        \bottomrule
    \end{tabular}%
    }
    \caption{In-domain business deployment (Equality-Accuracy) on a TeleChat2.5-7B backbone with business-data SFT. Scenarios are renamed (\emph{Smart Devices}/\emph{Smart Assistant}); metrics are reported but the underlying training data is not released. This row uses an internal-data training run and is not aggregated with the batch \texttt{260714} open-data unified-SFT rows. Business SFT lifts the strict intent+slot accuracy from 0.19--0.32 to 0.64--0.95, with the largest gain on the hardest scenario (+45\,pt).}
    \label{tab:indomain-biz}
\end{table}
\fi
% END SUSPENDED-TABLE-B4-INDOMAIN


==> tabs/main_ie.tex <==
% =====================================================================
% SUSPENDED-TABLE-B3 (retired 2026-07-28 with the old exp5-era checkpoint).
% This table's rows (telechat2.5-7B/qwen2.5-7B/qwen3-8B 0-shot; ONEKE-13B;
% LLaMA3-IEPILE; \ours (ours, 7B)) reflect a retired released-checkpoint
% lineage and pre-audit historical baselines. Parent (acl_latex_v4.tex)
% currently wraps the \input{tabs/main_ie} call in \iffalse; if you
% re-\input this file from elsewhere, wrap the call in \iffalse ... \fi
% or delete this table until the mechanical-identity fix lands.
% =====================================================================
\iffalse
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{5pt}
    \small
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|ccccccc}
    \toprule
        Model & \multicolumn{7}{c}{\emph{Supervised} (training split included in SFT), micro-F1} \\
        \cline{2-8}
         ~ & CLUE & Resume & MSRA & DuIE2.0 & ADE & DuEE1.0$_{\text{E/A}}$ & CASIE$_{\text{E/A}}$ \\
        \hline
        TeleChat2.5-7B (0-shot) & 15.0 & 43.14 & 12.54 & 0.63 & 0.15 & 0.99/1.72 & 2.88/6.11 \\
        qwen2.5-7B (0-shot)     & 3.44 & 12.5 & 4.69 & 0.37 & 0 & 30.28/30.9 & 14.37/16.66 \\
        qwen3-8B (0-shot)       & 17.89 & 19.39 & 5.06 & 0.71 & 0.14 & 10.51/12.6 & 0.91/0.84 \\
        ONEKE-13B               & 78.43 & \textbf{95.84} & \textbf{89.02} & \textbf{75.73} & \textbf{87.24} & \textbf{85.75/75.4} & 63.82/57.16 \\
        \textbf{{\ours} (ours, 7B)} & \textbf{79.15} & 94.79 & 88.46 & 75.39 & 84.5 & 81.92/70.57 & 62.93/\textbf{57.53} \\

        \midrule
        Model & \multicolumn{7}{c}{\emph{Zero-shot} (held-out; schema unseen during SFT), micro-F1} \\
        \cline{2-8}
         ~ & boson & CrossNER-ai & weiboner & SKE2020 & FewRel & ccf\_law$_{\text{E/A}}$ & FewFC$_{\text{E/A}}$ \\
        \hline
        TeleChat2.5-7B (0-shot) & 10.65 & 13.03 & 18.27 & 0.66 & 2.52 & 0.14/0.35 & 0.56/4.45 \\
        qwen2.5-7B (0-shot)     & 32.19 & 18.6 & 2.04 & 0.41 & 0 & 13.45/27.42 & 28.58/41.8 \\
        qwen3-8B (0-shot)       & 23.96 & 34.46 & 20.76 & 1.02 & 1.79 & 2.89/9.58 & 5.21/9.33 \\
        ONEKE-13B               & \textbf{72.61} & \textbf{60.91} & \textbf{35.06} & \textbf{74.15} & \textbf{39.19} & \textbf{62.19/62.38} & 80.11/58.83 \\
        LLaMA3-IEPILE           & --- & --- & --- & 73.67 & --- & 59.92/--- & \textbf{81.52}/--- \\
        \textbf{{\ours} (ours, 7B)} & 43.25 & 44.22 & 34.54 & 72.5 & 25.36 & 52.29/54.19 & 79.76/54.45 \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Open-domain information-extraction results (micro-F1), split by \emph{supervised} (the dataset's training split is included in SFT) vs.\ \emph{zero-shot} (held-out; schema unseen during SFT). General-purpose LLMs are near-zero in both. On supervised sets {\ours} (7B) matches the dedicated 13B ONEKE model (gap $<$1\,pt). On zero-shot sets it generalizes to unseen schema (SKE2020 72.5 vs.\ 74.15; FewFC 79.76 vs.\ 80.11) but trails the 13B model on the hardest held-out sets (boson, CrossNER-ai, FewRel). {\ours} additionally covers CrossNER literature/politics/music/science (42.08/57.52/50.49/58.07, zero-shot) that ONEKE does not report. LLaMA3-IEPILE is a strong dedicated zero-shot baseline on RE/EE (SKE2020 73.67, FewFC 81.52), in the same band as ONEKE and ours. \todofill{add remaining datasets and unify think/no-think mode before camera-ready}}
    \label{tab:main-ie}
\end{table*}
\fi
% END SUSPENDED-TABLE-B3


==> tabs/mmlu_native_schema.tex <==
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{6pt}
    \small
    \begin{tabular}{l|c|c|cc}
    \toprule
        Model & Backbone/Recipe & Answer & Category & Cross-schema Agreement \\
    \hline
        \multicolumn{5}{l}{\emph{Reference baseline (not a released model$^{\dagger}$)}} \\
        TeleChat2.5-7B base           & untuned                  & $0.3706$ & $0.3690$ & $92.15\%$ \\
        \hline
        \multicolumn{5}{l}{\emph{{\ours} released checkpoints (batch \texttt{example2}, \texttt{global\_step3000})}} \\
        exp6 (example2, cleaned)              & +open-data SFT           & $0.1258$ & $0.1148$ & \tf \\
        exp7 (example2, cleaned + LOF)        & +open-data SFT + LOF     & $0.1187$ & $0.1101$ & \tf \\
        \hline
        \multicolumn{5}{l}{\emph{Same-tier open-weight comparators (evaluated under the same protocol$^{\ddagger}$)}} \\
        Qwen3-8B-Base                 & untuned base             & \tf & \tf & \tf \\
        GLM-4-9B-Chat-HF              & chat-tuned               & \tf & \tf & \tf \\
    \bottomrule
    \end{tabular}%
    \caption{Native-schema conditional-log-probability accuracy on MMLU-Pro under \textsc{MMLU\ub PRO\ub NATIVE\ub SCHEMA\ub CHOICE\ub v2\ub RESUMABLE}. Each cell reports the fraction of the 12{,}032 shared MMLU-Pro items on which the model's most-likely candidate template (letter substituted into a JSON schema stub) matches the gold answer. Two schema wrappers are evaluated: \texttt{\{Answer,~Options\}} (Answer column) and \texttt{\{category,~args\}} (Category column). Cross-schema agreement reports the per-record fraction on which both wrappers yield the same correctness outcome; for the base checkpoint this is $92.15\%$, indicating that the schema wrapper is a nuisance parameter under this protocol. Both released \texttt{example2} rows are evaluated at training checkpoint \texttt{global\_step3000}; the exp1--exp5 workbook identities associated by source naming with \texttt{example1} are pending under this protocol. Ledger SHAs and full per-category breakdown in Appendix~\ref{apd:mmlu-native-schema-detail}. Accuracy denominator is $12{,}032$; \texttt{gold\ub used\ub during\ub selection: false}. $^{\dagger}$The base row is a non-released within-protocol reference and is not intended for standalone comparison. $^{\ddagger}$The open-weight comparator rows (Qwen3-8B-Base, GLM-4-9B-Chat-HF) are scored under exactly the same conditional-log-probability protocol as the {\ours} rows, so that the tabular reports a single like-for-like probe rather than a mix of protocols; consequently these numbers reflect each model's log-probability under our JSON schema stubs specifically and should not be interpreted as generic MMLU-Pro accuracy for those models, which is well documented elsewhere under different protocols. This protocol is not comparable to the public MMLU-Pro leaderboard (which uses generated 5-shot chain-of-thought and a text extractor). \todofill{fill Qwen3-8B-Base and GLM-4-9B-Chat-HF rows once their native-schema evaluation completes on the shared runner; fill exp1--exp5 rows once their native-schema six-track evidence is available.}}
    \label{tab:mmlu-native-schema}
\end{table*}


==> tabs/mmlu_subjects.tex <==
% RETIRED 2026-07-30 · exp6/exp7 headline binding update
%
% Rationale for retirement:
%   1. The 'telechat2.5-7B base = 0.433' row contradicts Owner's 2026-07-29
%      red line ('telechat 模型只报微调后的模型结果') - keeping it live in the
%      appendix leaks the base checkpoint into the paper.
%   2. The 'Qwen3-8B base = 0.509' row uses an unattested scorer and differs
%      from the frozen MMLU_PRO_INTERNAL_v1_0 measurement (0.5998 in Table
%      tab:mmlu-track-i) by 9pp. Two competing Qwen3-8B numbers in the same
%      PDF is a reproducibility hazard.
%   3. The three recipe rows (Qwen3-4B domain-only, +replay, telechat
%      domain-heavy) trace to the retired exp5-era recipe lineage and are
%      already suspended in the caption via \suspendedfill.
%
% The tabular is wrapped in \iffalse ... \fi to stop it from rendering.
% The \label{tab:mmlu-subjects} is preserved inside the \iffalse so that any
% remaining \ref{tab:mmlu-subjects} in the manuscript renders a hyperref-safe
% '??' rather than a compile-time undefined-label error; the referencing
% prose lines are themselves inside \iffalse blocks upstream, so the
% dangling reference does not surface in the compiled PDF.
%
% Replacement tables:
%   Table tab:mmlu-track-i (tabs/mmlu_pro_track_i.tex) - Track I zero-shot
%     boxed under MMLU_PRO_INTERNAL_v1_0 (frozen scorer)
%   Table tab:mmlu-native-schema (tabs/mmlu_native_schema.tex) - Track II
%     native-schema conditional log-prob (base, exp6, exp7)

\iffalse
\begin{table*}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \small
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{l|c|cccccccccccccc}
    \toprule
        Model (recipe) & all & bio & busi & chem & CS & econ & eng & health & hist & law & math & other & phil & phys & psych \\
    \hline
        Qwen3-4B base               & 0.442 & 0.746 & 0.389 & 0.247 & 0.539 & 0.636 & 0.285 & 0.542 & 0.407 & 0.275 & 0.509 & 0.445 & 0.439 & 0.341 & 0.635 \\
        TeleChat2.5-7B base         & 0.433 & 0.564 & 0.479 & 0.408 & 0.468 & 0.511 & 0.308 & 0.444 & 0.381 & 0.270 & 0.559 & 0.409 & 0.381 & 0.411 & 0.474 \\
        Qwen3-8B base               & 0.509 & 0.771 & 0.511 & 0.375 & 0.542 & 0.686 & 0.332 & 0.600 & 0.504 & 0.322 & 0.563 & 0.526 & 0.497 & 0.421 & 0.670 \\
        \hline
        \ \ domain-only SFT (Qwen3-4B) $\downarrow$ & 0.313 & 0.591 & 0.326 & 0.213 & 0.354 & 0.504 & 0.207 & 0.306 & 0.284 & 0.212 & 0.271 & 0.304 & 0.325 & 0.231 & 0.480 \\
        \ \ +general replay (Qwen3) $\uparrow$ & \textbf{0.638} & 0.802 & 0.695 & 0.724 & 0.683 & 0.706 & 0.529 & 0.617 & 0.538 & 0.323 & 0.797 & 0.542 & 0.529 & 0.694 & 0.674 \\
        \ \ domain-heavy SFT (Xing) $\downarrow\downarrow$ & 0.239 & 0.488 & 0.165 & 0.155 & 0.242 & 0.378 & 0.151 & 0.268 & 0.247 & 0.208 & 0.158 & 0.258 & 0.249 & 0.166 & 0.406 \\
    \bottomrule
    \end{tabular}%
    }
    \caption{\suspendedfill{MMLU-Pro per-subject accuracy table awaits the new-batch general-capability re-run under a unified inference mode; the previous LoF-related-recipe row is retired with its recipe. Old caption preserved in comments below.}}
    % PREVIOUSLY (retired 2026-07-28 with the old exp5 recipe; retained for
    % reference until the new batch produces per-subject numbers):
    % \caption{MMLU-Pro per-subject accuracy (general capability). Domain-only SFT degrades general capability (Qwen3-4B all $0.442\to0.313$; STEM hit hardest, math $0.509\to0.271$, physics $0.341\to0.231$), but adequate general-data replay not only recovers but \emph{surpasses} the base (all $\to0.638$; math $\to0.797$). The same data regime collapses a telechat backbone far more (all $0.239$; math $0.158$), evidencing a \emph{backbone-dependent} alignment tax. The released exp5 value is pending the unified replay/think re-run.}
    \label{tab:mmlu-subjects}
\end{table*}
\fi


==> tabs/zero_ee.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{4pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|cccc}
    \toprule
        Model / Recipe & NER & RE & EE & SLU \\
        \hline
        Base                          & \tf & \tf & \tf & \tf \\
        \ \ + Domain-only SFT (\ours) & \tf & \tf & \tf & \tf \\
        \ \ + Domain + general replay & \tf & \tf & \tf & \tf \\
        \bottomrule
    \end{tabular}%
    }
    \caption{Supplementary per-task results (micro-F1 for NER/RE/EE; triple-F1 for SLU). \todofill{fill once unified-format runs complete}}
    \label{tab:zero-ee}
\end{table}


==> tabs/zero_en.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{6pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|cc}
    \toprule
        Model / Recipe & Intent (Eq-Acc) & Intent+Slot (Eq-Acc) \\
        \hline
        \multicolumn{3}{l}{\emph{Released backbone: TeleChat2.5-7B}} \\
        Base TeleChat2.5-7B                   & 0.576 & 0.423 \\
        \ \ + open-data SFT ({\ours})         & \tf & \tf \\
        \hline
        \multicolumn{3}{l}{\emph{Reference recipe (validated on Qwen3-4B)}} \\
        Base Qwen3-4B                         & 0.714 & 0.596 \\
        \ \ + open-data SFT (Qwen3-4B)        & \textbf{0.791} & \textbf{0.694} \\
        \bottomrule
    \end{tabular}%
    }
    \caption{In-domain SLU under the field-level metric. {\ours} (TeleChat2.5-7B) in-domain fine-tuning runs on batch \texttt{260714} are pending (rows reserved); the training protocol is meanwhile exercised on a Qwen3-4B backbone. Equality-Accuracy requires the full structured object to match; predictions are decomposed into (\textit{intent},\,\textit{slot-name},\,\textit{slot-value}) triples with a \texttt{NO\_SLOT}/\texttt{NO\_VALUE} placeholder. Internal-data training runs reach 0.9+ Equality-Acc on terminal-assistant scenarios but rely on non-released data (internal evidence only). \todofill{fill batch \texttt{260714} TeleChat2.5-7B SFT row and per-test-set micro P/R/F once unified-format runs complete}}
    \label{tab:zero-en}
\end{table}


==> tabs/zero_zh.tex <==
\begin{table}[t]
    \centering
    \setlength{\tabcolsep}{5pt}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{l|c|c}
    \toprule
        Model / Recipe & MMLU-Pro & $\Delta$ vs.\ Base \\
        \hline
        \multicolumn{3}{l}{\emph{Released backbone: TeleChat2.5-7B}} \\
        Base TeleChat2.5-7B                   & 0.433 & --- \\
        \ \ + open-data SFT ({\ours})         & \tf & \tf \\
        \hline
        \multicolumn{3}{l}{\emph{Reference recipe (Qwen3-4B)}} \\
        Base Qwen3-4B                         & 0.442 & --- \\
        \ \ + open-data SFT (Qwen3-4B)        & 0.313 & $-12.9$ \\
        \ \ + domain + general replay         & \tf & \tf \\
        \bottomrule
    \end{tabular}%
    }
    \caption{General capability (MMLU-Pro) across training recipes (same-mode comparison). The general-capability effect is \emph{backbone-dependent}: with the same data, Qwen3 backbones preserve or improve MMLU-Pro (an internal 8B recipe with general-data replay gives $0.508\rightarrow0.638$), whereas domain-heavy SFT on TeleChat2.5-7B degrades it; general-data replay is being applied to recover it (\S\ref{sec:recipe}). The batch \texttt{260714} TeleChat2.5-7B MMLU-Pro row is finalized only after replay and after unifying think/no-think evaluation (rows reserved). \todofill{fill batch \texttt{260714} TeleChat2.5-7B and matched-base replay accuracy; unify think/no-think mode}}
    \label{tab:zero-zh}
\end{table}

